Statistical Privacy

To analyze the privacy guarantee of personal data in a database that is subject to queries it is necessary to model the prior knowledge of a possible attacker. Differential privacy considers a worst-case scenario where he knows almost everything, which in many applications is unrealistic and requires a large utility loss. This paper considers a situation called statistical privacy where an adversary knows the distribution by which the database is generated, but no exact data of all (or sufficient many) of its entries. We analyze in detail how the entropy of the distribution guarantes privacy for a large class of queries called property queries. Exact formulas are obtained for the privacy parameters. We analyze how they depend on the probability that an entry fulfills the property under investigation. These formulas turn out to be lengthy, but can be used for tight numerical approximations of the privacy parameters. Such estimations are necessary for applying privacy enhancing techniques in practice. For this statistical setting we further investigate the effect of adding noise or applying subsampling and the privacy utility tradeoff. The dependencies on the parameters are illustrated in detail by a series of plots. Finally, these results are compared to the differential privacy model.

==> 250227_StatisPrivacy <==
\begin{thebibliography}{10}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\providecommand{\doi}[1]{https://doi.org/#1}

\bibitem{ACG16}
Abadi, M., Chu, A., Goodfellow, I., McMahan, H., Mironov, I., Talwar, K.,
  Zhang, L.: Deep learning with differential privacy. In: Proc.~ACM CC. pp.
  308--318 (2016)

\bibitem{BBG20}
Balle, B., Barthe, G., Gaboardi, M.: Privacy profiles and amplification by
  subsampling. J.~Privacy and Confidentiality  \textbf{10}(1) (2020).
  \doi{10.29012/jpc.726}

\bibitem{BGKS13}
Bassily, R., Groce, A., Katz, J., Smith, A.: Coupled-worlds privacy: Exploiting
  adversarial uncertainty in statistical data privacy. In: Proc.~54.~FOCS. p.
  439–448 (2013). \doi{10.1109/FOCS.2013.54}

\bibitem{BBG11}
Bhaskar, R., Bhowmick, A., Goyal, V., Laxman, S., Thakurta, A.: Noiseless
  database privacy. In: Proc.~ASIACRYPT 2011. pp. 215--232. Springer LNCS 7073
  (2011)

\bibitem{D21}
Desfontaines, D.: A list of real-world uses of differential privacy.
  https://desfontain.es/blog/real-world-differential-privacy.html (2021)

\bibitem{DMK20}
Desfontaines, D., Mohammadi, E., Krahmer, E., Basin, D.: Differential privacy
  with partial knowledge (2020)

\bibitem{DP22}
Desfontaines, D., Pejo, B.: Sok: Differential privacies -- a taxonomy of
  differential privacy variants and extensions (2022)

\bibitem{DMN16}
Dwork, C., McSherry, F., Nissim, K., Smith, A.: Calibrating noise to
  sensitivity in private data analysis. J.~Privacy and Confidentiality
  \textbf{3},  17--51 (2016)

\bibitem{DR14}
Dwork, C., Roth, A.: The algorithmic foundations of differential privacy.
  Foundations and Trends® in Theoretical Computer Science  \textbf{9}(3–4),
  211--407 (2014). \doi{10.1561/0400000042}

\bibitem{IC21}
Imola, I., Chaudhuri, K.: Privacy amplification via {Bernoulli} sampling. In:
  Proc.~38.~Int.~Conf.~on Machine Learning (2021)

\bibitem{JD22}
Joseph, N., David, D.: Differential privacy: Future work \& open challenges.
  https://www.nist.gov/blogs/cybersecurity-insights/differential-privacy-future-work-open-challenges
  (1 2022), an official website of the United States government

\bibitem{KL12}
Kifer, D., Lin, B.: An axiomatic view of statistical privacy and utility.
  J.~Privacy and Confidentiality  \textbf{4},  5--49 (2012)

\bibitem{M18}
Meiser, S.: Approximate and probabilistic differential privacy definitions.
  Cryptology ePrint Archive (2018)

\bibitem{M17}
Mironov, I.: Renyi differential privacy. In: Proc.~30.~Computer Security
  Foundations Symposium (2017)

\bibitem{SMM19}
Sommer, D., Meiser, S., Mohammadi, E.: Privacy loss classes: The central limit
  theorem in differential privacy. In: Proc.~Privacy Enhancing Technologies
  Symposium. vol. 2019 (2), pp. 245--269 (2019). \doi{10.2478/popets-2019-0029}

\bibitem{S22}
Steinke, T.: Composition of differential privacy and privacy amplification by
  subsampling. In: arXiv:2210.00597 (2022)

\bibitem{WBK19}
Wang, Y., Balle, B., Kasiviswanathan, S.: Subsampled {Renyi} differential
  privacy and analytical moments accountant. In: Proc.~22.~AISTATS (2019)

\end{thebibliography}

